DeepWear: Adaptive Local Offloading for On-Wearable Deep Learning

Due to their on-body and ubiquitous nature, wearables can generate a wide range of unique sensor data creating countless opportunities for deep learning tasks. We propose DeepWear, a deep learning (DL) framework for wearable devices to improve the performance and reduce the energy footprint. DeepWear strategically offloads DL tasks from a wearable device to its paired handheld device through local network. Compared to the remote-cloud-based offloading, DeepWear requires no Internet connectivity, consumes less energy, and is robust to privacy breach. DeepWear provides various novel techniques such as context-aware offloading, strategic model partition, and pipelining support to efficiently utilize the processing capacity from nearby paired handhelds. Deployed as a user-space library, DeepWear offers developer-friendly APIs that are as simple as those in traditional DL libraries such as TensorFlow. We have implemented DeepWear on the Android OS and evaluated it on COTS smartphones and smartwatches with real DL models. DeepWear brings up to 5.08X and 23.0X execution speedup, as well as 53.5% and 85.5% energy saving compared to wearable-only and handheld-only strategies, respectively.

==> section/biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/xumengwei}}]{Mengwei~Xu}
is a Ph.D student in the School of Electronics Engineering
and Computer Science of Peking University, Beijing, China.  His research interests include mobile computing and operating system.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/feng}}]{Feng~Qian}
is an assistant professor in the Computer Science and Engineering Department at the University of Minnesota -- Twin Cities. His research interests cover the broad areas of mobile systems, VR/AR, computer networking, and system security.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.25in,clip,keepaspectratio]{figure/bio/Mengze}}]{Mengze~Zhu} is an undergraduate student in the School of Electronics Engineering
and Computer Science of Peking University, Beijing, China. His research interests include Mobile Systems and Machine Learning.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.25in,clip,keepaspectratio]{figure/bio/Feifan}}]{Feifan~Huang} is an undergraduate student in the School of Electronics Engineering
and Computer Science of Peking University, Beijing, China. His research interests include Mobile Systems and Machine Learning.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1.2in,height=1.25in,clip,keepaspectratio]{figure/bio/Saumay}}]{Saumay~Pushp}is a Ph.D candidate in the School of Computing, Korea Advanced Institute of Science and Technology, Daejeon, South Korea. His research interests include Mobile Systems and Networking.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/Xuanzhe}}]{Xuanzhe~Liu}
is an associate professor in the School of Electronics Engineering
and Computer Science, Peking University, Beijing, China. His research interests
are in the area of services computing, mobile computing, web-based systems, and big data analytics. He is the corresponding author of this work.
\end{IEEEbiography} 
